Scavenger: A Cloud Service for Optimizing Cost and Performance of ML Training

While the pay-as-you-go nature of cloud virtual machines (VMs) makes it easy to spin-up large clusters for training ML models, it can also lead to ballooning costs. The 100s of virtual machine sizes provided by cloud platforms also makes it extremely challenging to select the ``right'' cloud cluster configuration for training. Furthermore, the training time and cost of distributed model training is highly sensitive to the cluster configurations, and presents a large and complex tradeoff-space. In this paper, we develop principled and practical techniques for optimizing the training time and cost of distributed ML model training on the cloud. Our key insight is that both parallel and statistical efficiency must be considered when selecting the optimum job configuration parameters such as the number of workers and the batch size. By combining conventional parallel scaling concepts and new insights into SGD noise, our models accurately estimate the time and cost on different cluster configurations with < 5% error. Using the repetitive nature of training and our models, we can search for optimum cloud configurations in a black-box, online manner. Our approach reduces training times by 2 times and costs more more than 50%. Compared to an oracle-based approach, our performance models are accurate to within 2% such that the search imposes an overhead of just 10%.

==> bg.tex <==
\section{Background}
\label{sec:bg}

In this section we look at distributed ML training and the tradeoffs involved in scaling it in data center and cloud environments. 



\subsection{Cloud Resource Selection}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> intro.hpdc.tex <==

% Clearly state the objective of the paper and provide (quantitative) support to motivate the specific problem your submission is solving.
\paragraph{Motivation}

%    . Briefly review the most relevant and most recent prior works. Clearly articulate the limitations of prior works and how your approach breaks away from those limitations. A more detailed discussion should be reserved for the related work section. But, this section should be sufficient to help readers recognize the novelty of your approach.
\paragraph{Limitation of state-of-art approaches}

%    Key insights and contributions. Briefly articulate the major insights that enable your approach or make it effective. Clearly specify the novelty of these insights and how they advance state-of-the-art. Describe the key ideas of your approach and design. List the key contributions including flagship empirical results and improvement over the prior art as applicable.

\paragraph{Key insights and contributions}

%     Experimental methodology and artifact availability. Clearly specify the key experimental / simulation infrastructure and methodological details. Support the experimental methodology choices (e.g., cite that most relevant and most recent prior works have evaluated their ideas using similar methodology). Include a line to indicate whether the software/hardware artifact will be available upon acceptance.

\paragraph{Experimental methodology and artifact availability}

%     Limitations of the proposed approach. Almost all scientific contributions have limitations and scope for improvement. Clearly articulate all the major limitations of the proposed approach and identify conclusions that are sensitive to specific assumptions made in the paper.

\paragraph{Limitations}
  
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> intro2.tex <==
\section{Introduction}
\label{sec:intro}

Machine learning models are increasingly being trained on distributed clusters in data centers and clouds.
ML model training requires a large amount of computational resources, and the

Cost vs. time tradeoff is fundamental due to a large number of reasons. First is regular Amdahl scaling laws due to the periodic communication.
Second is the batch size which not only affects the parallel scaling (the number of iterations and communication overhead can be reduced by increasing the batch size).
But larger batches introduce other statistical efficiency considerations.
The total training time is determined by \emph{both} parallel and statistical efficiency.
The batch size also affects the \emph{cost} of training because of the larger machines and GPUs required for larger batches.


\begin{enumerate}
\item We examine the parallel and statistical efficiency tradeoff in SGD-driven data-parallel training.
\item We show how statistical efficiency can be used in a performance model to predict the running time for various cluster and batch sizes. 
\end{enumerate}

==> pareto-alloc.tex <==
\section{Resource Allocation and Scaling}

Cluster selection can be done for different objective functions, depending on the user requirements:
\begin{enumerate}
\item Deadline 
\item Budget
\item Knee point based 
\item General optimization of cost and time 
\end{enumerate}

For each case we note that constraints on K, B are essential. These constraints also inferred during the optimization search phase.
Search strategy is guided by 

As shown in \S\ref{sec:eval}, the compute cost and training time follows a pareto frontier \cite{mccandlish2018empirical}.  We evaluate different cost functions where we assume statically priced VMs as well as pricing VMs based on the amount of computation they perform (which in turn depends on a workers' mini-batch size $b$).
Over all the possible allocations in the defined $kspace$, \textit{KneePtSearch} function applies a \emph{KneePoint} search \cite{kneedle} to find the inflection point corresponding to the configuration that best balances the trade-off between cost and time. Thus, for each $\mathit{B}$, we get a configuration after applying the kneepoint search. For multiple $\mathit{B}_{new}$ in Algo. \ref{alg:scaling-algo}, we thus get various optimal $(\mathit{K},\mathit{B})$  configs.  Of all the kneepoint configs, we choose the config that minimizes the (cumulative cost $\times$ time).

General technique: 
Knee-finding: 2nd derivative, curvature. 
Perturb and observe with stochastic hillclimbing.
Coordinate descent and line-search on either K or B depending on the constraints and the knobs? For each K, find the B* and then select the best for the custom tradeoff option.
For Pareto optimal: again, depending on budgets, determine the 

Can support either or both. 

Perturb and update performance model parameters and estimate total time and cost.
For aiding the line-search: extreme points prefered: thus very small and large K for each B. 


Two major scenarios of deployment:
1. If the full tradeoff curves are known, this is simple.
2. Do this purely online.

\noindent \textbf{Perturb and update perf model.} Using the performance model from (\ref{eqn:normnoise-epochs}) and (\ref{eqn-noise-rootB}), predict the noise and epochs for the new configuration. The $\textit{LogIterationTime}$ function involves running invoking Tensorflows' \cite{tensorflow} forward and backward propagation to log the gradient computation and synchronization time. The overhead of running a model and logging iteration time is minimal since we only do it for a few iterations (typically running 10-20 steps and taking average). Knowing the estimated epochs and iteration time, we can predict the total training time taken and compute cost using eqns. (\ref{eqn:time-model},\ref{eqn:cost-model}). 

\begin{comment}
Next, we extend the offline performance model described above and approximate the same for online adjustment in Scavenger's scaling algorithm. In Algo. \ref{alg:scaling-algo}, we describe the scaling technique to select the \textit{best available $(\mathit{K},\mathit{B})$ configuration, while still considering the statistical inefficiency in SGD training and parallel inefficiency imposed by Amdahl's law}. Here, the \textit{best available configuration} is one that minimizes (cost $\times$ time). Based on the selected $(\mathit{K},\mathit{B})$ and availability of resources, we scale the workers up or down and resume training with the updated worker count using checkpoint-restart technique.

The user defines the bounds on the global batch size to use in distributed training by setting $\mathit{B}_{min}$ and $\mathit{B}_{max}$ respectively.
We start training with an initial configuration of $(\mathit{K}_{min},\mathit{B}_{min})$ and log the noise (normalized by $\mathit{K}_{min}$) and epochs taken, once the former has stabilized. Repeat the same for the configuration $(\mathit{K}_{min},\mathit{B}_{max})$, and fit the results in eqn (\ref{eqn:normnoise-epochs}). Similarly, we fit noise and corresponding global batch size used in eqn. (\ref{eqn-noise-rootB}).Then, we explore various $(\mathit{K}_{new},\mathit{B}_{new})$ configurations by adjusting parameters $bspace$ and $kspace$, such that $\mathit{K}_{new} \in [\mathit{K}_{min},\mathit{K}_{max}]$ and $\mathit{B}_{new} \in [\mathit{B}_{min},\mathit{B}_{max}]$.  As static or transient resources are added or revoked \cite{awsspot,gcppremptible}, we dynamically adjust $\mathit{K}_{min}$ and $\mathit{K}_{max}$ accordingly to predict time and cost of the new configurations, and select one that minimizes both.


%There are models to estimate these times as well \cite{qiao2021pollux}, but they only hold true for a predetermined compute hardware in the cluster and not workers with varying compute capabilities.  The overhead of running the ML model and logging time is minimal since we only do it for a few iterations. Knowing the estimated epochs and iteration time, we can predict the total training time taken and compute cost using (\ref{eqn:time-model},\ref{eqn:cost-model}).

%\SetAlgoLined
\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\SetKwFunction{LogNoiseEpoch}{LogNoiseEpoch}
\SetKwFunction{LogIterationTime}{LogIterationTime}\SetKwFunction{KneePtSearch}{KneePtSearch} 
\SetKwFunction{FitNoiseB}{FitNoiseB}
\SetKwFunction{FitNoiseEpoch}{FitNoiseEpoch} \SetKwFunction{Randint}{randint}
\SetKwFunction{Range}{range} 
\Input{$\mathit{K_{\mathit{min}}}, \mathit{B_{\mathit{min}}}, \mathit{K_{\mathit{max}}}, \mathit{B_{\mathit{max}}}, \mathit{bspace}, \mathit{kspace}$}
\Output{$(\mathit{K}_{\mathit{ideal}}, \mathit{B}_{\mathit{ideal}})$ config to minimize cost-time}
\BlankLine
$\mathit{D} \leftarrow$ total training data samples\\
$\mathit{perVMcost} \leftarrow$ hourly \$ cost of one worker\\
$(\mathit{n}_{1}, \mathit{e}_{1})$ $\leftarrow$ \LogNoiseEpoch{$\mathit{K}_{min}$, $\mathit{B}_{min}$}\;
$(\mathit{n}_{2}, \mathit{e}_{2})$ $\leftarrow$ \LogNoiseEpoch{$\mathit{K}_{min}$, $\mathit{B}_{max}$}\;
$\mathit{fitting1}$ $\leftarrow$ \FitNoiseB{$[\mathit{n}_{1},\mathit{n}_{2}], [\mathit{B}_{min},\mathit{B}_{max}]$}\;
$\mathit{fitting2}$ $\leftarrow$ \FitNoiseEpoch{$[\mathit{n}_{1},\mathit{n}_{2}], [\mathit{e}_{1},\mathit{e}_{2}]$}\;
$\mathit{timecost} \leftarrow dict()$\\
$\mathit{idealconf} \leftarrow dict()$\\
\For{ i $\leftarrow$ \Range{$\mathit{bspace}$}} {
$\mathit{B}_{new} \leftarrow$ \Randint{$\mathit{B}_{\mathit{min}},\mathit{B}_{\mathit{max}}$}\\
\For{ i $\leftarrow$ \Range{$\mathit{kspace}$}} {
$\mathit{K}_{new} \leftarrow$ \Randint{$\mathit{K}_{\mathit{min}},\mathit{K}_{\mathit{max}}$}\\
$\mathit{noise}_{new} \leftarrow \mathit{fitting1.predict(\mathit{B}_{new})}$\\
$\mathit{epochs}_{new} \leftarrow \mathit{fitting2.predict(\mathit{noise}_{new})}$\\
$\mathit{itr} \leftarrow$ \LogIterationTime{$\mathit{K}_{new}, \mathit{B}_{new}$}\;
$pred\_iterations \leftarrow (\mathit{D} \times \mathit{epoch}_{new})/\mathit{B}_{new}$\\
$est\_time \leftarrow (\mathit{itr} \times \mathit{pred\_iterations})$\\
$cost \leftarrow (K_{new} \times \mathit{est\_time} \times \mathit{perVMcost})$\\
$\mathit{timecost}[est\_time, cost] \leftarrow (\mathit{K}_{new}, \mathit{B}_{new})$\\
}
$\mathit{time} \leftarrow list(timecost.keys[0])$\\
$\mathit{cost} \leftarrow list(timecost.keys[1])$\\
$\mathit{t}_{knee}, \mathit{c}_{knee} \leftarrow$ \KneePtSearch{$\mathit{time}$, $\mathit{cost}$}\\
$(\mathit{K}_{knee}, \mathit{B}_{knee}) \leftarrow timecost.get(\mathit{t}_{knee}, \mathit{c}_{knee})$\\
$\mathit{idealconf}[\mathit{t}_{knee}\times\mathit{c}_{knee}] \leftarrow (\mathit{K}_{knee}, \mathit{B}_{knee})$\\
}
\BlankLine
\BlankLine
$\mathit{min\_timecost} \leftarrow \mathbf{min.} \mathit{idealconf.keys()}$\\
$(\mathit{K}_{ideal}, \mathit{B}_{ideal}) \leftarrow \mathit{idealconf.value(\mathit{min\_timecost})}$
\BlankLine
\KwRet{$(\mathit{K}_{ideal}, \mathit{B}_{ideal})$}
%\BlankLine
%\BlankLine
\caption{Online Scavenger Scaling}\label{alg:scaling-algo}
\end{algorithm}
\DecMargin{1em}
\end{comment}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> policies.tex <==
\section{Scaling Policies}

\subsection{Pareto Frontiers}

\subsection{Weighted cost and time}

\subsection{}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> skel.tex <==

\section{BG}

\subsection{Data parallel training}

\subsection{Parallel Scaling}
Add workers
Increase batch size
Time and cost in the cloud 

\section{Performance Model of parallel and statistical scaling}

Parallel scaling amadahl

Statistical efficiency vs. batch sizes

Gradient noise definition 

Modeling the number of epochs E(K,B) using empirical Gradient noise 


\section{Resource Selection Policy}

\section{Implementation}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> tradeffs.tex <==

\section{Challenges and Tradeoffs in Distributed Training}

\textbf{Introduce the main concepts here? Workers, batch-size, tput, TTA.}


\begin{figure*}
  \subfloat[ResNet18 \label{fig:cluster-scaling}]
  {\includegraphics[width=0.3\textwidth]{clusterscaling.pdf}}	
  \subfloat[Transformer \label{fig:memory-limit}]
  {\includegraphics[width=0.3\textwidth]{transformemlimitfail.pdf}}
  \subfloat[ResNet18 \label{fig:loss-steps-examples}]
  {\includegraphics[width=0.3\textwidth]{resnet18lossitregs.pdf}}
  \caption{(a) Improvement in training time as cluster size and capacity scales. ResNet18, ResNet50 and Transformer Tiny are run upto 80\% train acc. on CIFAR-10,90\% on CIFAR-100 and 15.0 BLEU on WMT14 dataset. (b) Training Accuracy reached by Transformer Base config before job failed due to memory constraints. (c) Training time and examples taken by ResNet18 on CIFAR-10 to converge.  \textit{Larger $\mathit{B}$ are more time efficient to reach the same loss.}}
	\label{fig:mergebgplots}
\end{figure*}


Distributed training is resource \emph{elastic}, which means that the same model can be trained using multiple parallelism levels, which can also happen to be dynamic.
This elasticity is well matched with the cloud: since different types of VMs can be added.

Distributed training has complex and ill-understood trade-offs between parallel efficiency, synchronization overheads, and the quality of the trained model.
Like most parallel applications, adding more workers and increasing the parallelism has diminishing returns due to the periodic parameter synchronization (Amdahl's law \cite{yavits2013effect}). However, additional scaling considerations apply.


Two key scaling knobs. The first is the number of workers, $K$, which can be achieved by provisioning and using more virtual machines (VMs).
This increases the parallelism.


\subsection{Horizontal Scaling: Workers}
\label{subsec:amdahl}

\emph{Work-scaling} can be achieved by increasing the global or total batch size, which increases the work done per-step and reduce the synchronization overhead.
\emph{Thus, we can respond to resource availability changes by changing the number of workers and adjusting the batch size and hence the total work performed. }
However, the batch size has many subtle trade-offs with the statistical efficiency and model quality. With large batch sizes, there are diminishing returns in training time due to the stochastic nature of the SGD noise.

There are numerous factors governing the training time and cost of running a ML model like the computing capability of the individual workers, synchronization costs (due to network bandwidth, location of workers on same/different racks or data centers), optimization used (Nestrov, Momentum, Adam,RMSProp etc.), learning rate, and other hyperparameters. In essence, they are specific to a training job, and must be learned on the fly. Thus, there is a limit to how far we should ideally increase the global batch size. Thus, given the aforementioned factors, there is an ideal batch size that balances the trade-off between the running time and cost. In  \S\ref{sec:design}, we develop techniques to infer scalability characteristics by using signals from the optimization process, and use it for developing scaling policies.

Fig. \ref{fig:compute-sync-time} shows the scaling limitations across various cluster size $K$ and global batch size $B$ configurations for different ML workloads. 
The synchronization time increases with the cluster size as gradients from  more workers need to be reduced on the parameter servers, reducing the effective bandwidth. 
Here, the cumulative cluster capacity is same across various $\mathit{K}$, i.e., total CPU cores and memory allocated over all the workers in a cluster is same regardless of the cluster size. The iteration time also increases for any $\mathit{B}$ as $\mathit{K}$ increases even though worker mini-batch size decreases.  This happens because the per-worker compute capacity decreases as $K$ keeps increasing.
For example, if all clusters have total $96$vCPUs and $96$GB memory for ResNet18 workload, then clusters with $(8,12,16)$ workers have per-worker compute config of $(12,8,6)$vCPUs and $(12,8,6)$GB memory. The worker mini-batch size for global batch size of $768$ is $(96,64,48)$ but the iteration times are $(1.45,1.55,1.64)$ sec. respectively. Thus, iteration time increases even though worker mini-batch size decreases on increasing cluster size when cumulative cluster capacity is the same.

\begin{figure*}
		\hspace{1.5cm}
		%\centering
		\subfloat[ResNet18 \label{fig:resnet18-computesynctime}]
  		{\includegraphics[width=0.3\textwidth]{resnet18clustersametime.pdf}}	
  		\subfloat[ResNet50 \label{fig:resnet50-computesynctime}]
  		{\includegraphics[width=0.3\textwidth]{resnet50clustersametime.pdf}}
  		\subfloat[Transformer Base \label{fig:transformer-computesynctime}]
  		{\includegraphics[width=0.3\textwidth]{transformerclustersametime.pdf}}

	\caption{The gradient computation and synchronization time breakdown for various ML workloads across multiple $K$ and trained on various $\mathit{B}$ with PS strategy. The cumulative cluster capacity is same across all $\mathit{K}$.}
	\label{fig:compute-sync-time}
\end{figure*}



When increasing the number of workers we further have a choice.
The is to keep global batch size B fixed, in which case the per-worker mini-batch size decreases with increasing K, since b=B/k.
This can reduce the gradient computation time and result in shorter iterations.



One way is to increase the number of workers computing the gradients.
This provides easy way to 

Distributed training is important as it boosts up the training process by adding more workers and increasing the amount of work done per-unit of time. The gains of increasing cluster size by adding more workers in data-parallel training with PS can be seen in Fig. \ref{fig:cluster-scaling} for various workloads.

Different ML models require a bare minimum hardware to run effectively. While CPUs and GPUs determine the pace of the training, the memory available to such models (esp. models like Transformers, RNN etc.) and the massive datasets they train on determine the extent of convergence before the job terminates due to resource constraints. Fig. \ref{fig:memory-limit} shows this, as observed on our private compute cluster \cite{futuresystems}. Various distributed training approaches \cite{sergeev_horovod:_2018, li_scaling_2014} address these constraints by distributing training on more compute nodes and using larger global batch sizes.

However, distributed training faces challenges like significant communication and synchronization overhead due to model update at every step, implying \emph{parallel inefficiency}, and reducing the effectiveness of parallel scaling. But unlike other parallel applications, data-parallel training has other \emph{statistical efficiency} tradeoffs influenced by the number of workers and the batch size. As we explain in more detail in \S\ref{subsec:dml-tradeoff}, scaling in distributed ML cannot be analyzed with just Amdahl's law \cite{yavits2013effect} due to the statistical inefficiency in SGD optimization.


\subsection{Vertical Scaling: Batch Size}

Training models on large global batch sizes increases the compute efficiency of the individual workers due to larger per-worker batch size. Thus, more samples can be trained per-unit of time and converge a model in lesser time.  For $K=16$, the training time to convergence on the three ML workloads is shown in Fig. \ref{fig:time-multipleB}. ResNet18, ResNet50 and Transformer Base are trained to 80\%,90\% training accuracy and 18.0 BLEU score respectively. The training time decreases as $B$ increases.

\begin{figure}[H]
\hspace*{-0.4cm} 
\includegraphics[width=0.52\textwidth]{workloadstimebatchsize.pdf}
\caption{Training time to convergence for various global batches on $\mathit{K=16}$.  ResNet18, ResNet50 and Transformer Base are converged to 80\%, 90\% training accuracy and 18.0 BLEU score respectively.}
\label{fig:time-multipleB}
\end{figure}

\begin{figure}[H]
\hspace*{-0.3cm}
\includegraphics[width=0.52\textwidth]{throughputB.pdf}
\caption{Throughput of various models on increasing the global batch size B for $\mathit{K=16}$. The throughput increases as we increase $\mathit{B}$ upto a certain point, then plateaus.}
\label{fig:throughput-B}
\end{figure}


The gains of compute efficiency with larger $B$ is evident from Fig. \ref{fig:throughput-B} where the throughput (i.e., the number of samples processed per second in the training phase) increases as the global batch size increases, then saturates after a knee-point/inflection point. The throughput plateaus after a certain batch size since the CPU utilization of the workers maxed out after the inflection point. In the results shown, the workers used in the cluster are GCP E2-standard VMs with 4vCPUs and 16GB memory.

Worker with higher compute units could increase the throughput as well as the global batch size corresponding to the inflection point. Nevertheless, it is still bounded by the parallel scaling limitations of the individual workers as governed by Amdahl's law, and shown in \S\ref{subsubsec:amdahl}.

The gains of using larger batches are further bolstered by the results in Fig. \ref{fig:loss-steps-examples}.  Larger $\mathit{B}$ can achieve the same loss value in lesser training iterations,  implying smaller training time when run on the same hardware configuration. Thus, larger batches are more time efficient.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Statistical inefficiency and Gradient Noise}
\label{subsec:statsineff}

Fundamental reason for the non-linear scaling is that not all computing work is effective because of stochastic gradient descent.
There is statistical inefficiency which we must capture.

Need to explain fundamental reason for inefficiency very clearly.
Parallel workers. Gradient updates in different directions. More workers means more divergence. Smaller batches also mean more approximate gradients. So larger batches are better. But require memory, and have diminishing returns, as we also show, supported by prior work.


In Full Gradient Descent (FGD), the model iterates over the entire training dataset to compute the gradients  and update model parameters at each training iteration. In FGD, model arrives at the minima directly and convergence is relatively smooth. However, training progress is slow at each step on account of the exorbitant computational requirements to train on entire dataset at every iteration. On the other hand, in Stochastic Gradient Descent (SGD) the model computes the gradients and updates parameters on a single sample at a time. SGD is especially useful when the dataset is colossal. Still, SGD can be slow as well since a single training example cannot be vectorized for faster execution. Mini-Batch Gradient Descent (Mini-Batch GD) merges the best of both worlds between FGD and SGD where a model trains on a mini-batch to compute gradients and update model parameters at every step.

As we go from FGD $\rightarrow$ Mini-Batch GD $\rightarrow$ SGD (in the order of decreasing batch size), statistical inefficiency reduces the progress made towards convergence for a given unit of work (number of data samples processed during model training). The main cause of this inefficiency is the stochastic nature of the optimization process. With Mini-Batch GD and SGD, the computed gradients become less representative of the true gradient computed with FGD. The gradients in Mini-Batch GD and SGD have higher variance than the true gradient in FGD. Thus, the gradients are noisy when computed on a \textit{mini-batch}. We say \textit{mini-batch} because SGD can also be looked as a variation of Mini-Batch GD with mini-batch size $1$. With smaller batches, the gradient variance is greater, and increasing the batch size can reduce the noise and thus increase the overall progress made in each iteration. 

% below repeated somewhere exactly

However, increasing the  batch size too much would result in diminishing statistical efficiency. Larger batch sizes have lower noise and increasing it beyond a certain point would \emph{not} result in any notable noise reduction. This means extra computations are performed which do not contribute towards the model convergence. Our goal is to find this batch size threshold for a given cluster size beyond which scaling the application does not reduce the training time significantly (i.e., the knee-point).
The SGD noise, which can be approximated as the variance between the gradients, can be used to find such a threshold. We demonstrate the impact of noise on the training time and epochs to convergence in \S\ref{sec:design}. We also show how to readily compute the noise by looking at the computed gradients prior and post aggregation in data-parallel training strategy \cite{mccandlish2018empirical,johnson2020adascale}.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

